Extraction of Salient Sentences from Labelled Documents

We present a hierarchical convolutional document model with an architecture designed to support introspection of the document structure. Using this model, we show how to use visualisation techniques from the computer vision literature to identify and extract topic-relevant sentences. We also introduce a new scalable evaluation technique for automatic sentence extraction systems that avoids the need for time consuming human annotation of validation data.

==> discussion.tex <==
%!TEX root = txtnets_nips2014.tex

\section{Discussion}

Overfitting. Dear god the overfitting.



==> tikz_layer_drawing_macros.tex <==
% The angles of x,y,z-axes
\newcommand\xaxis{0}
\newcommand\yaxis{30}
\newcommand\zaxis{90}

\def\layer[#1,#2,#3][#4][#5][#6]{
    % [1:x,2:y,3:z][4:width][5:depth][6:name]
    \coordinate[
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ] (#6-sw) at (0,0);
    \coordinate[
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ] (#6-se) at (#5,0);
    \coordinate[
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ] (#6-nw) at ($(\yaxis:#4)$);
    \coordinate[
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ] (#6-ne) at ($(\yaxis:#4) + (#5,0)$);

    % outline
    \draw[
    draw=black, 
    ultra thick,
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ]
    (0,0) -- ++ (\xaxis:#4) -- ++ (\yaxis:#5) -- ++ (\xaxis:-#4) -- cycle;

    % vertical bars
    \foreach \xx in {1,...,#4}
    {
      \draw[
      	draw=gray,
      	thin,
	    shift={(\xaxis:#1)},
	    shift={(\yaxis:#2)},
	    shift={(\zaxis:#3)}
	    ]
	    ($(\xaxis:\xx)$) -- ++ (\yaxis:#5);
    }

    % horizontal bars
    \foreach \y in {1,...,#5}
    {
      \draw[
      	draw=gray,
      	thin,
	    shift={(\xaxis:#1)},
	    shift={(\yaxis:#2)},
	    shift={(\zaxis:#3)}
	    ]
	    ($(\yaxis:\y)$) -- ++ (\xaxis:#4);
    }
}



\def\layerconnector[#1,#2,#3][#4,#5][#6,#7,#8][#9]{
	% [x,y,z][height,width] for begin then [x,y,z] for end (always 1x1)
	% 9 = color

	% bottom
    \fill[
    fill=#9!20,
    fill opacity=0.5,
    draw=#9,
    very thick,
    shift={(\xaxis:#1)},
    shift={(\yaxis:#2)},
    shift={(\zaxis:#3)}
    ]
    (0,0) -- ++ (\xaxis:#5) -- ++ (\yaxis:#4) -- ++ (\xaxis:-#5) -- cycle;

    % top
    \fill[
    fill=#9!20,
    fill opacity=0.5,
    draw=#9, 
    very thick,
    shift={(\xaxis:#6)},
    shift={(\yaxis:#7)},
    shift={(\zaxis:#8)}
    ]
    (0,0) -- ++ (\xaxis:1) -- ++ (\yaxis:1) -- ++ (\xaxis:-1) -- cycle;

    % connector edges
    \draw[
    draw=#9,
    very thick
    ]
    % front left
    ($(\xaxis:#1) + (\yaxis:#2) + (\zaxis:#3)$) -- ($(\xaxis:#6) + (\yaxis:#7) + (\zaxis:#8)$)
    % front right
    ($(\xaxis:#1+#5) + (\yaxis:#2) + (\zaxis:#3)$) -- ($(\xaxis:#6+1) + (\yaxis:#7) + (\zaxis:#8)$)
    % back left
    ($(\xaxis:#1) + (\yaxis:#2+#4) + (\zaxis:#3)$) -- ($(\xaxis:#6) + (\yaxis:#7+1) + (\zaxis:#8)$)
    % back right
    ($(\xaxis:#1+#5) + (\yaxis:#2+#4) + (\zaxis:#3)$) -- ($(\xaxis:#6+1) + (\yaxis:#7+1) + (\zaxis:#8)$)
    ;
}

